Search-based Automated Program Repair of CPS Controllers Modeled in Simulink-Stateflow

Stateflow models are widely used in the industry to model the high-level control logic of Cyber-Physical Systems (CPSs) in Simulink--the defacto CPS simulator. Many approaches exist to test Simulink models, but once a fault is detected, the process to repair it remains manual. Such a manual process increases the software development cost, making it paramount to develop novel techniques that reduce this cost. Automated Program Repair (APR) techniques can significantly reduce the time for fixing bugs by automatically generating patches. However, current approaches face scalability issues to be applicable in the CPS context. To deal with this problem, we propose an automated search-based approach called FlowRepair, explicitly designed to repair Stateflow models. The novelty of FlowRepair includes, (1) a new algorithm that combines global and local search for patch generation; (2) a definition of novel repair objectives (e.g., the time a fault remained active) specifically designed for repairing CPSs; and (3) a set of mutation operators to repair Stateflow models automatically. We evaluated FlowRepair with three different case study systems and a total of nine faulty stateflow models. Our experiments suggest that (1) Flo wRepaircan fix bugs in stateflow models, including models with multiple faults; (2) FlowRepair surpasses or performs similarly to a baseline APR technique inspired by a well-known CPS program repair approach. Besides, we provide both a replication package and a live repository, paving the way towards the APR of CPSs modeled in Simulink.

==> ResultsTable.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\centering
\caption{Summary of the results for each mutant (10 different repetitions) when deployed in operation (physical testing) or in off-line.}
\label{table:TimeResults}
\scriptsize
\resizebox{\textwidth}{!}{\begin{tabular}{cr|rrrrrrr|rrrrrrr|}
\cline{3-16}
\multicolumn{1}{l}{}                                & \multicolumn{1}{l|}{}                       & \multicolumn{7}{c|}{\textbf{Physical Testing}}                                                                                                                                                                                                                                                                                                          & \multicolumn{7}{c|}{\textbf{Off-line Testing}}                                                                                                                                                                                                                                                                                                          \\ \cline{3-16} 
\multicolumn{1}{l}{}                                & \multicolumn{1}{l|}{}                       & \multicolumn{3}{c|}{\textbf{Linear Speed}}                                                                            & \multicolumn{3}{c|}{\textbf{Angular Speed}}                                                                           & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Mutant \\ Killed\end{tabular}}}} & \multicolumn{3}{c|}{\textbf{Linear Speed}}                                                                            & \multicolumn{3}{c|}{\textbf{Angular Speed}}                                                                           & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Mutant \\ Killed\end{tabular}}}} \\ \cline{2-8} \cline{10-15}
\multicolumn{1}{l|}{}                               & \multicolumn{1}{l|}{\textbf{Configuration}} & \multicolumn{1}{r|}{\textbf{Killed}} & \multicolumn{1}{r|}{\textbf{p-val}}    & \multicolumn{1}{r|}{\textbf{d-cohen}} & \multicolumn{1}{r|}{\textbf{Killed}} & \multicolumn{1}{r|}{\textbf{p-val}}    & \multicolumn{1}{r|}{\textbf{d-cohen}} & \multicolumn{1}{c|}{}                                                                                   & \multicolumn{1}{r|}{\textbf{Killed}} & \multicolumn{1}{r|}{\textbf{p-val}}    & \multicolumn{1}{r|}{\textbf{d-cohen}} & \multicolumn{1}{r|}{\textbf{Killed}} & \multicolumn{1}{r|}{\textbf{p-val}}    & \multicolumn{1}{r|}{\textbf{d-cohen}} & \multicolumn{1}{l|}{}                                                                                   \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{HLR}}} & LR = 0.0001                                      & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.2544}            & \multicolumn{1}{r|}{-0.5265}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.2878}            & \multicolumn{1}{r|}{-0.4899}          & False                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{0.001}             & \multicolumn{1}{r|}{1.727}            & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{0.0003}            & \multicolumn{1}{r|}{1.9820}           & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & LR = 0.0002                                      & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.2660}            & \multicolumn{1}{r|}{-0.5134}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.2878}            & \multicolumn{1}{r|}{-0.4899}          & False                                                                                                       & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.062}             & \multicolumn{1}{r|}{0.889}            & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{0.0053}            & \multicolumn{1}{r|}{1.4175}           & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & LR = 0.0005                                      & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.5187}            & \multicolumn{1}{r|}{-0.2944}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.5560}            & \multicolumn{1}{r|}{-0.2683}          & False                                                                                                       & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.510}             & \multicolumn{1}{r|}{0.301}            & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.9411}            & \multicolumn{1}{r|}{0.0335}           & False                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & LR = 0.005                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-2.4083}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-2.5298}          & True                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{0.008}             & \multicolumn{1}{r|}{1.330}            & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{0.0316}            & \multicolumn{1}{r|}{1.0426}           & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & LR = 0.01                                        & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-4.0018}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-4.0249}          & True                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{44.0822}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{38.8273}          & True                                                                                                       \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{TAN}}} & PoP = 5\%                                        & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.5220}            & \multicolumn{1}{r|}{-0.2920}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.5560}            & \multicolumn{1}{r|}{-0.2683}          & False                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{0.010}             & \multicolumn{1}{r|}{1.2977}           & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{0.0006}            & \multicolumn{1}{r|}{-1.8504}          & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & PoP = 0.1\%                                         & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.9467}            & \multicolumn{1}{r|}{-0.0303}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{1}                 & \multicolumn{1}{r|}{0.0000}           & False                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{0.001}             & \multicolumn{1}{r|}{1.7995}           & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.4304}            & \multicolumn{1}{r|}{-0.3607}          & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & PoP = 0.15\%                                        & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.9561}            & \multicolumn{1}{r|}{0.0249}           & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{1}                 & \multicolumn{1}{r|}{0.0000}           & False                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{2.2397}           & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{0.0033}            & \multicolumn{1}{r|}{1.5150}           & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & PoP = 0.2\%                                         & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.8409}            & \multicolumn{1}{r|}{-0.0911}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.5560}            & \multicolumn{1}{r|}{-0.2683}          & False                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{2.9245}           & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{5.0658}           & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & PoP = 25\%                                        & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.2593}            & \multicolumn{1}{r|}{-0.5209}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.1346}            & \multicolumn{1}{r|}{-0.7006}          & False                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{4.7084}           & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{7.6013}           & True                                                                                                       \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{TCL}}} & PoI = 15\%                                        & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-2.5252}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-2.5298}          & True                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{11.7770}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{16.4045}          & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & PoI = 2\%                                      & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-4.0018}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-4.0249}          & True                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{13.9346}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{15.5744}          & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & PoI = 25\%                                        & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-4.0018}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-4.0249}          & True                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{19.8078}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{13.8662}          & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & PoI = 3\%                                         & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-4.0018}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-4.0249}          & True                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{12.2734}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{18.3378}          & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & PoI = 35\%                                        & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-4.0018}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{-4.0249}          & True                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{15.0016}          & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{16.9399}          & True                                                                                                       \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{HNE}}} & NoE = 2                                           & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.3208}            & \multicolumn{1}{r|}{-0.4566}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.1346}            & \multicolumn{1}{r|}{-0.7006}          & False                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{4.8816}           & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{6.4894}           & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & NoE = 5                                           & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.2680}            & \multicolumn{1}{r|}{-0.5112}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.2878}            & \multicolumn{1}{r|}{-0.4899}          & False                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{4.4124}           & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{3.8986}           & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & NoE = 8                                           & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.2419}            & \multicolumn{1}{r|}{-0.5412}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.2878}            & \multicolumn{1}{r|}{-0.4899}          & False                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{3.0027}           & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{\textless{}0.0001} & \multicolumn{1}{r|}{2.3360}           & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & NoE = 12                                          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.2478}            & \multicolumn{1}{r|}{-0.5342}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.2878}            & \multicolumn{1}{r|}{-0.4899}          & False                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{0.0004}            & \multicolumn{1}{r|}{1.9242}           & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.0808}            & \multicolumn{1}{r|}{0.8275}           & True                                                                                                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                              & NoE = 15                                          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.0563}            & \multicolumn{1}{r|}{-0.9124}          & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.0544}            & \multicolumn{1}{r|}{-0.9204}          & False                                                                                                       & \multicolumn{1}{r|}{True}               & \multicolumn{1}{r|}{0.0190}            & \multicolumn{1}{r|}{1.1526}           & \multicolumn{1}{r|}{False}               & \multicolumn{1}{r|}{0.1359}            & \multicolumn{1}{r|}{0.6982}           & True                                                                                                       \\ \hline
\end{tabular}}
\end{table*}

